Beyond Model Interpretability: On the Faithfulness and Adversarial Robustness of Contrastive Textual Explanations

Contrastive explanation methods go beyond transparency and address the contrastive aspect of explanations. Such explanations are emerging as an attractive option to provide actionable change to scenarios adversely impacted by classifiers' decisions. However, their extension to textual data is under-explored and there is little investigation on their vulnerabilities and limitations. This work motivates textual counterfactuals by laying the ground for a novel evaluation scheme inspired by the faithfulness of explanations. Accordingly, we extend the computation of three metrics, proximity,connectedness and stability, to textual data and we benchmark two successful contrastive methods, POLYJUICE and MiCE, on our suggested metrics. Experiments on sentiment analysis data show that the connectedness of counterfactuals to their original counterparts is not obvious in both models. More interestingly, the generated contrastive texts are more attainable with POLYJUICE which highlights the significance of latent representations in counterfactual search. Finally, we perform the first semantic adversarial attack on textual recourse methods. The results demonstrate the robustness of POLYJUICE and the role that latent input representations play in robustness and reliability.

==> constrastive_formulation_notworking.tex <==
\textbf{Definition 1 (Counterfactual Explanation)} \textit{Assuming a predictor, potentially non-linear, $f: \mathcal{X} \mapsto \mathcal{Y}$, an instance $\bm{x^i} \in \mathcal{X}$ such that $f(\bm{x^i}) = y_{\text{fact}}$ and a foil class $y_{\text{foil}}$, a counterfactual $\bm{x}_{cf}^i \in \mathcal{X}$ can be computed by:}
\begin{align}
    \underset{\bm{x}_{cf}}{\arg \min} & d(\bm{x}_{cf}^i , \bm{x^i})\\
    \text{subject to} & f(\bm{x}_{fl}^i) =  y_{\text{foil}}
\end{align}\label{eq:formulation}
where $d(.)$ is a distance metric. This optimization can be also perceived as 
\begin{equation}
    \underset{\bm{x}_{cf}}{\arg \min} \hspace{1em} L(f(\bm{x}_{fl}^i), y_{\text{foil}}) + \lambda d(\bm{x}_{cf}^i , \bm{x^i})
\end{equation}
in the Lagrangian notation, with $l(.)$ denoting a loss function and $\lambda>0$ is a regularization factor that balances the minimal edit distance (through minimizing the distance between the factual and the counterfactual) and the success rate (by finding a counterfactual that successfully changes the model's decision). 

% assumptions on f
Depending on the method, restrictions and assumptions might complement the above definition. For instance, model-specific recourse methods \cite{ustun2019actionable} put assumptions on $f$ whereas model-agnostic ones assume a black-box architectures \cite{poyiadzi2020face,joshi2019towards}. 


% distance
When considering the counterfactual cost or distance $d(.)$, the literature has formed a consensus on the use of the (normalized) $l_0$ or $l_1$ norm or any convex combination thereof \cite{mothilal2020explaining,karimi2020model,ustun2019actionable,wachter2017counterfactual}. In some cases, a simple Euclidean distance measure is an oversimplification of the underlying application complexity which might lead to distorted counterfactuals based on their data distribution. Accordingly, research in ExAI community is witnessing a momentum in the direction of considering manifold-like distance measures. Some approaches \cite{zhou2021cdl,dosovitskiy2016generating,larsen2016autoencoding} employ adversarial learning to non-linearly model latent spaces \cite{goodfellow2014generative}. Other approaches \cite{INACIO2021407,ishfaq2018tvae,samanta2020vae,joshi2019towards} use Variational Auto-Encoders (VAEs) \cite{kingma2014auto} to removing low-density regions in the latent space which allows the counterfactuals to satisfy attainability \cite{pawelczyk2021carla}.


% search --> GD, graph search, growing spheres
Different methods are devised to solve the optimization problem above. One line of research deploys gradient-based techniques to achieve a feasible solution \cite{dhurandhar2018explanations,mothilal2020explaining,schut2021generating}. Another track focuses on graph search techniques \cite{poyiadzi2020face}, growing hyper-spheres \cite{laugel2017inverse} and integer programming tools \cite{ustun2019actionable}. Some methods \cite{mothilal2020explaining} add a diversity constraint on the search paradigm promoting a diverse counterfactual set. 

Interested readers are referred to \cite{survey} and \cite{karimi2020survey} that survey state-of-the-art methods on algorithmic recourse methods. 
